PMNet: Robust Pathloss Map Prediction via Supervised Learning

Pathloss prediction is an essential component of wireless network planning. While ray tracing based methods have been successfully used for many years, they require significant computational effort that may become prohibitive with the increased network densification and/or use of higher frequencies in 5G/B5G (beyond 5G) systems. In this paper, we propose and evaluate a data-driven and model-free pathloss prediction method, dubbed PMNet. This method uses a supervised learning approach: training a neural network (NN) with a limited amount of ray tracing (or channel measurement) data and map data and then predicting the pathloss over location with no ray tracing data with a high level of accuracy. Our proposed pathloss map prediction-oriented NN architecture, which is empowered by state-of-the-art computer vision techniques, outperforms other architectures that have been previously proposed (e.g., UNet, RadioUNet) in terms of accuracy while showing generalization capability. Moreover, PMNet trained on a 4-fold smaller dataset surpasses the other baselines (trained on a 4-fold larger dataset), corroborating the potential of PMNet.

==> Table/Coverage.tex <==
\begin{tabularx}{1\linewidth}{l c c}
\toprule[1pt]
{Dataset} & Exclusive (Small) & Exclusive \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}
mIOU & $???$ \% \; & $???$ \%
\\
\bottomrule[1pt]
\end{tabularx}





==> Table_Parameter.tex <==
\begin{table}[t!]\footnotesize
	\vspace{.5em}
	\centering
	\caption{Simulation parameters.}
	\resizebox{\columnwidth}{!}{\begin{tabular} {l l}
			%\begin{tabular} {P{1.4cm} P{0.001cm} P{0.001cm} P{0.001cm} P{0.001cm}P{0.001cm} P{0.001cm}}
			\toprule[1pt]
			\textbf{Parameter} & \textbf{Value} \\
			\midrule
			Time slot size & $\delta_t=10$  \\
			Number of time slot for a episode & $N=513$ \\
			\multirow{2}{*}{Positions of Src and Dst} & $\mathbf{q}_{\mathcal{S}}=[0,0,0]^T$, \\  
			& $\mathbf{q}_{\mathcal{D}}=[4000,4000,0]^T$ \\
			Altitude of SAT & $H_{\mathrm{L}}=550$ {[}km{]} (from \cite{Starlink}) \\ 
			Velocity of SAT\footnotemark & $\mathbf{v}_{\mathrm{L}, \mathrm{I}}=[0, 7.8, 0]^T$ {[}km/s{]} \\
			Radius of orbital plane & $r_{\mathrm{E}} = 6921$ {[}km{]} \\ 
			Length of orbital plane & $c_{\mathrm{E}} = 43486$ {[}km{]} \\ 
			Number of SAT in orbital plane & $I = 22$ \\ 
			Distance between satellites & $1976$ {[}km{]}  \\
			Length of plane in coordinate space & $c_{\mathrm{C}} = 4000$ {[}km{]} \\ 
			Number of SAT in coordinate space & $I' = 2$ \\ 
			Bandwidth for RF link & $B_{\mathrm{RF}} = 10^{9}$ {[}Hz{]} \\   
			Reference SNR ($d=1$ {[}m{]}), Path-loss exponent & $\gamma_{0} = 10^{9}$, $\alpha = 2$ \\ 
			Learning rate, Discount factor & 0.0001, 0.95 \\ 
			Batch size, \# of iterations/update & 500, 500 \\ 
			Training iterations & 500000 \\
			\bottomrule[1pt]
	\end{tabular}}
	\label{table_Paramter}
	\vspace{-1.6em}  
\end{table} 

==> omer/background_cnn_omer.tex <==
In the realm of supervised learning, it's known to all that CNN's are the go-to networks for image tasks, due to its lower computation with less nodes compared to Fully-connected networks.

we have the following prediction for the true label $y_i \in \mathbb{R}^m$:
\begin{equation}
    \hat{y}_i \triangleq \sigma\big(W_k\dots \sigma(W_2\sigma(W_1\overline{\boldsymbol{x}}_i))\big)
\end{equation}
where $W_k$ is the weight matrix for the layer $k \in \{1, 2, \dots, K \}$ We also have $\overline{\boldsymbol{x}}_i = [1\;\boldsymbol{x}_i]^T$, where $\boldsymbol{x}_i \in \mathbb{R}^n$ is the input feature vector of the neural network. One may observe that number of parameters computations are growing $\mathcal{O}(K \times m \times n)$, which can be quite expensive and computationally intractable. On the other hand, Convolutional Neural Network(CNN) brings a solution to this memory and computational cost problem of deep and high dimensional cases\cite{lecun}. In addition to computational problem, fully connected networks lacks of equivariant representation and such as translation in time-series data or local translation image classification which requires poor performance results over the test sets \cite{deep_book}.

A standard CNN consists of convolution layer, non-linear activation function, pooling and a fully-connected layer. 
The number of layers for each type of layer might be different. 
The convolutional layer uses filters or kernels $h(i, j)$ to apply 2-D convolutional operation to the input feature $\boldsymbol{x} \in \mathbb{R}^{m \times n}$ as shown below: 
\begin{equation}
    z_{i,j} = \sum_{m = 1}\sum_{n = 1} h_{i - m, j - n}\vb*{x}_{m, n}
\end{equation}
After the convolutional layer, a nonlinear function is applied which leads to the feature maps. Moreover, as the kernels are smaller than the input features, than the corresponding feature maps would be smaller than the input features.This structure is called as sparse interactions \cite{deep_book}. In addition to decreasing the dimensions as the same kernel is used also helps to memory considerations as it allows to share the parameters along the convolution procedure. Finally, pooling layer is applied which also reduction of the dimension, while preserving local information in the features \cite{deep_book}.




Aforementioned properties of CNNs are the backbones many widely used architectures and models. CNNs show tremendous result in image classification with models AlexNet \cite{alexnet}, VGG \cite{VGG} and ResNet\cite{resnet}. Image segmentation employs CNN for medical cases with U-Net shown in \cite{ref:UNet}. Aside the real-life application, CNNs are also used in statistical method to generate more data to feed deep neural networks as an augmentation method \cite{dcgan}.





==> omer/background_radiounet_fadenet.tex <==
RadioUNet \cite{ref:RadioUNet} and FadeNet \cite{ref:Fadenet} are two models, which employ U-Nets for PMP. We look at the U-Net architectures, datasets, training procedures,  and the experimental setup they have used. In terms of U-Net architectures, RadioUNet uses two cascaded U-Nets creating a W-Net as they call it. Individual U-Nets in RadioUNet sticks to the original U-Net \cite{ref:UNet} architecture with 18 convolutional layers and different filter sizes.  FadeNet uses single UNet with 28 convolutional layers and the filter sizes varies over the model.

% Once we created the architecures, we may discuss the datasets. RadioUnet uses city maps with and without cars, the transmitter location and a sub-sampled radio map in gray scale as their input features. They use Dominant Path Model(DPM) and Intelligent Ray Tracing (IRT) as their ground truth or label generator and convert generated radio maps onto the interval 0 and 1, namely gray scale. On the other hand, FadeNet uses city maps again but with terrain, building, foliage heights maps and also a binary map for Line Of Sight(LOS) paths from locations on the map to the base station. As ground truth for the dataset, they LSF maps in dB generated via Ray Tracing(RT) tool. Moreover, FadeNet employs data augmentation techniques to enlarge their dataset and increase transferability capabilities. 

RadioUnet employs curriculum learning, where they first train the first UNet, then train the the second UNet by feeding the same inputs and also the outputs of the first UNet. They employ Normalized Mean Square Error(NMSE) and Root Mean Square Error(RMSE) as their performance metric. They train on a dataset which contains input features as city map and Tx locations and another scenario which consists an additional feature cars and using fine IRT-4 data in their input features. FadeNet uses RMSE as their loss and they do scenarios with input features like city map, terrain, building, foliage heights maps and with or without a binary map for Line Of Sight(LOS) paths from locations. Additionally, they present generalizability examples where they in train the network in one city and test it in another city. 

==> omer/background_unet.tex <==
% In the previous section, we gave UNet as a model employing CNNs in medical image segmentation. Here, we are going to go deeper to understand architecture of UNets. 
UNets build their architetures upon two fundamental structures, autoencoders(AE)\cite{auteoncoders} and CNNs. AEs are neural networks which aim to find a latent space that represents the data in a smallar space. Thus, AEs are widely used in dimensionality reduction \cite{dim_redux} and generative modeling \cite{vae}. UNets uses autoencoder architecture as their backbone with respect to UNets' encoding and decoding parts. The modification that UNets are making is feeding the decoder de-convolution layers with the corresponding outputs of the convolutional layers in the encoder. 

Similar tools used in CNNs such as convolutional and pooling layers can be seen in the architecture. On the other hand, they do not employ any fully connected layers. In addition to that, in the decoder part they use upsampling/deconvolution operator to increase resolution back. Traditionally CNNs are used to classify the image as a whole, but UNets make pixel-wise classification to get the desired semantic  segmentation.  



==> repo/abstract_omer.tex <==
As the demand for better and faster communication increases, accurate pathloss prediction gains more importance. Having measurements or making model-based predictions could be a viable solution. However, these methods are not always possible to apply or they would not be accurate enough. As a solution, we present a data driven method to predict pathloss from a given terrain map. The method makes the pathloss prediction problem model free and easily accesible as terrain maps can be gathered freely. In this work, we introduce PMNet, which employs atrous convolution and hourglass network. The proposed algorithm achieves state of art results in terms of prediction and generalization capabilities. PMNet outperforms RadioUNet by from \% 20 to 29\%  decrease in normalized mean square error(NMSE). 

==> repo/background_cnn_omer.tex <==
In the realm of supervised learning with fully connected neural networks, we have the following prediction for the true label $y_i \in \mathbb{R}^m$:
\begin{equation}
    \hat{y}_i \triangleq \sigma\big(W_k\dots \sigma(W_2\sigma(W_1\overline{\boldsymbol{x}}_i))\big)
\end{equation}
where $W_k$ is the weight matrix for the layer $k \in \{1, 2, \dots, K \}$ We also have $\overline{\boldsymbol{x}}_i = [1\;\boldsymbol{x}_i]^T$, where $\boldsymbol{x}_i \in \mathbb{R}^n$ is the input feature vector of the neural network. One may observe that number of parameters computations are growing $\mathcal{O}(K \times m \times n)$, which can be quite expensive and computationally intractable. On the other hand, Convolutional Neural Network(CNN) brings a solution to this memory and computational cost problem of deep and high dimensional cases\cite{lecun}. In addition to computational problem, fully connected networks lacks of equivariant representation and such as translation in time-series data or local translation image classification which requires poor performance results over the test sets \cite{deep_book}.

A standard CNN consists of convolution layer, non-linear activation function, pooling and a fully-connected layer. The number of layers for each type of layer might be different. The convolutional layer uses filters or kernels $h(i, j)$ to apply 2-D convolutional operation to the input feature $\boldsymbol{x} \in \mathbb{R}^{m \times n}$ as shown below: 
\begin{equation}
    z(i,j) = \sum_{m = 1}\sum_{n = 1} h(i - m, j - n)\boldsymbol{x}(m, n)
\end{equation}
After the convolutional layer, a nonlinear function is applied which leads to the feature maps. Moreover, as the kernels are smaller than the input features, than the corresponding feature maps would be smaller than the input features.This structure is called as sparse interactions \cite{deep_book}. In addition to decreasing the dimensions as the same kernel is used also helps to memory considerations as it allows to share the parameters along the convolution procedure. Finally, pooling layer is applied which also reduction of the dimension, while preserving local information in the features \cite{deep_book}.

Aforementioned properties of CNNs are the backbones many widely used architectures and models. CNNs show tremendous result in image classification with models AlexNet \cite{alexnet}, VGG \cite{VGG} and ResNet\cite{resnet}. Image segmentation employs CNN for medical cases with U-Net shown in \cite{ref:UNet}. Aside the real-life application, CNNs are also used in statistical method to generate more data to feed deep neural networks as an augmentation method \cite{dcgan}.


==> repo/background_radiounet_fadenet_omer.tex <==
RadioUNet \cite{ref:RadioUNet} and FadeNet \cite{ref:Fadenet} are two models, which employ U-Nets for RMP. We look at the U-Net architectures, datasets, training procedures,  and the experimental setup they have used. In terms of U-Net architectures, RadioUNet uses two cascaded U-Nets creating a W-Net as they call it. Individual U-Nets in RadioUNet sticks to the original U-Net \cite{ref:UNet} architecture with 18 convolutional layers and different filter sizes.  FadeNet uses single UNet with 28 convolutional layers and the filter sizes varies over the model.

Once we created the architecures, we may discuss the datasets. RadioUnet uses city maps with and without cars, the transmitter location and a sub-sampled radio map in gray scale as their input features. They use Dominant Path Model(DPM) and Intelligent Ray Tracing (IRT) as their ground truth or label generator and convert generated radio maps onto the interval 0 and 1, namely gray scale. On the other hand, FadeNet uses city maps again but with terrain, building, foliage heights maps and also a binary map for Line Of Sight(LOS) paths from locations on the map to the base station. As ground truth for the dataset, they LSF maps in dB generated via Ray Tracing(RT) tool. Moreover, FadeNet employs data augmentation techniques to enlarge their dataset and increase transferability capabilities. 

RadioUnet employs curriculum learning, where they train the first UNet firstly, then train the the second UNet by feeding with the same inputs and also the outputs of the first UNet. They employ Normalized Mean Square Error(NMSE) and Root Mean Square Error(RMSE) as their performance metric. The scenarios they used is having cars or not and using fine IRT-4 data in their input features. FadeNet uses RMSE as their loss and they do scenarios with or without LOS input feature. Additionally, they present generalizability examples where they in train the network in one city and test it in another city. 

==> repo/background_unet_omer.tex <==
In the previous section, we gave UNet as a model employing CNNs in medical image segmentation. Here, we are going to go deeper to understand architecture of UNets. UNets build their architetures upon two fundamental structures, autoencoders(AE)\cite{auteoncoders} and CNNs. AEs are neural networks which aim to find a latent space that represents the data in a smallar space. Thus, AEs are widely used in dimensionality reduction \cite{dim_redux} and generative modeling \cite{vae}. UNets uses autoencoder architecture as their backbone with respect to UNets' encoding and decoding parts. The modification that UNets are making is feeding the decoder de-convolution layers with the corresponding outputs of the convolutional layers in the encoder. 

The tools used from CNNs in  such as convolutional and pooling layers. On the other hand, they do not employ any fully connected layers in the architecture. Moreover, in the decoder part they use upsampling/deconvolution operator to increase resolution back. Moreover, traditionally CNNs are used to classify the image as a whole, yet UNets makes pixel-wise classification to get the desired semantic  segmentation.  



==> repo/conclusion_omer.tex <==
In this article, we introduced a state of art method, PMNet, for pathloss map prediction. PMNet leverages the recent image segmentation techniques such as atrous convolution and hourglass networks. The performance of PMNet is evaluated in terms of NMSE and GNL. We showed that PMNet outperforms vanilla UNet and RadioUNet both in prediction accuracy and generalization capabilities. As a real life application of the pathloss prediction, we demonstrated that how PMNet's predictions can be employed in covarage prediction with respect to different thresholds.

==> repo/intro_omer.tex <==
% The essence of Radio Map Prediction(RMP) is the estimation of a certain location's propagation path loss through a model with or without a set of measurements(data). We start introducing RMP methods in the case of the absence of any measurements. In such cases, the only thing we have in our hands is the model, which is constructed through propagation physics. \cite{ray_tracing} employs ray tracing, and \cite{dominant} employs the dominant path model as their model and uses their model to find out the path loss at each location. The downside of such models is the coarse assumptions, which might not be extended in real-world applications.
Radio map prediction (RMP) estimates a certain location's propagation path loss through a model with or without a set of measurement data. 

The model-based RMP, which uses no measurement data, is the one example which is based on a physical principle for wireless propagation. In particular, \cite{ray_tracing} employs ray tracing, and \cite{dominant} employs the dominant path model as its model and uses their model to find out the path loss at each location.
In such cases, it is only based on coarse assumptions, which might not apply to an actual network environment.


% Going one step further from not having any data, we may have measurements at some locations of interest. There are ways of inducing the measurements to predict the propagation path loss in locations such that the measurement does not exist. The existing measurements are used to tune the physical model parameters; then, interpolation models are employed for locations without measurement. In \cite{voronoi}, the authors used Log-Distance Path Loss (LDPL) as a propagation model and a Voronoi tessellation-based method for the interpolation. Moreover, in \cite{slf} Spatial Loss Field(SLF) is used as a path loss model, and the low-rank, sparse matrix structure of SLF is exploited for interpolation purposes. 
Going one step further from \emph{without} data to \emph{limited} data, there are ways of inducing the measurements to predict the propagation path loss in locations where the measurement does not exist, using a limited measurement dataset for some locations of interest. 
The limited measurement data are used to tune the physical model parameters; then, interpolation models are employed for locations without measurement. 
In \cite{voronoi}, the authors used log-distance path loss (LDPL) as a propagation model and a Voronoi tessellation-based method for the interpolation. Moreover, in \cite{slf} spatial loss field (SLF) is used as a path loss model, and the low-rank, sparse matrix structure of SLF is exploited for interpolation purposes. 



% The underlying physical phenomenon is the challenging part of the problem solution in the methods above. Due to the lack of data, the model's accuracy is quite important in representing physical reality. On the other hand, we may exploit the data structure for the interpolation even without a physical model, but with a parametric linear model such as linear regression, \cite{survey_radiomap}, where basis functions are the distance from the measurement point to the transmitters. Moreover, kernel-based methods let the user pick a kernel, which removes the search for physically meaningful basis functions \cite{kernel}. Methods like kriging in \cite{kriging} just uses the statistical properties of the measured data, whereas tensor completion \cite{tensor_completion} and compressed sensing \cite{compressed_sensing} based methods employ the structure of the collected data.
On the other side, there is another way for RMP that focus more on the limited data in terms of statistics. 
Even without a physical model, the limited data itself can be exploited for interpolation with a parametric linear model, such as linear regression \cite{survey_radiomap}.
\tredd{
[Please put a more general (high-level) explanation for linear regression, kernel, and kriging.  ]
}

% Up to this point, we employed propagation physics as a prior, interpolation methods with respect to data structure and collection methodology, and statistical properties of the measured data. Yet, we would like to create mappings from different features of the measurement locations, such as a city map, building structure, etc. The reason behind this goal is to have generalizable models that allow us to get rid of the laborious data collection phase and models that do not match with the real-world application. Deep learning brings us the flexibility of using different input features to have such mappings for RMP. In \cite{ref:RadioUNet} and \cite{cnn} authors uses city maps as their input feature to have RMP. Moreover, in \cite{ref:Fadenet}, authors have used terrain, building, and foliage heights in addition to city maps for their input features of deep neural networks. 
Up to this point, we discuss several RMP methods using the physical principle as a prior, \tredd{XXX}, and the statistical properties of the measured data. However, those methods are somewhat limited to predicting the channel over the map with no measurement data; some are not precise enough, and others require measurement data at least a little bit.
Measurement data is expensive in terms of time and computing resources; thus, only a limited number of data can be utilized.
That calls for a model that can more precisely predict a channel condition over a large-scale map with no prior information.
Deep learning provides a clue to solving such demands for the RMP method.
In \cite{ref:RadioUNet} and \cite{ref:Fadenet}, authors leveraged computer-vision-oriented deep neural network architecture and used topographic information (e.g., terrain, building, and foliage heights) as their input feature for RMP. 





  
% In addition to the generalization capability and finding mappings from different input features to the radio maps, neural networks can be used to transfer the knowledge as shown in \cite{transfer_learning_radiomap}, which allows us to use the same neural networks without costly training procedure. Finally, performance-wise, the deep learning methods are successful too, where the transformer method in \cite{transformer_radiomap} achieves higher validation scores than mentioned methods.
